BiT: Robustly Binarized Multi-distilled Transformer

Modern pre-trained transformers have rapidly advanced the state-of-the-art in machine learning, but have also grown in parameters and computational complexity, making them increasingly difficult to deploy in resource-constrained environments. Binarization of the weights and activations of the network can significantly alleviate these issues, however, is technically challenging from an optimization perspective. In this work, we identify a series of improvements that enables binary transformers at a much higher accuracy than what was possible previously. These include a two-set binarization scheme, a novel elastic binary activation function with learned parameters, and a method to quantize a network to its limit by successively distilling higher precision models into lower precision students. These approaches allow for the first time, fully binarized transformer models that are at a practical level of accuracy, approaching a full-precision BERT baseline on the GLUE language understanding benchmark within as little as 5.9%. Code and models are available at: https://github.com/facebookresearch/bit.

==> Binary Transformer (3)/backup/submission_supplementary_backup.tex <==
\section{Appendix}

\subsection{\ours{} vs. Progressive Distillation}\label{sec:progressive_ablation}
\input{tables/progressive}
Previous work has also recognized the importance of good initialization for binary model training, and proposed to perform distillation while progressively quantizing the student model \citep{zhuang2018towards, yang2019synetgy}.  Progressive distillation ensures a good initialization for the student model at each step.  However, in this approach the teacher model is fixed to the full precision model, which does not address the problem of teacher-student gap.  In Table \ref{tab:progressive} we compare \ours{} to a comparable implementation of progressive distillation, using the same quantization schedule, W32A32 $\rightarrow$ W1A2 $\rightarrow$ W1A1, as ours.  We keep the teacher model fixed, while re-initializing the student model from the latest quantized version at each step.  We see that using a quantized teacher model is helpful, especially in the high-data regime. However, our method can lag behind progressive distillation for small datasets such as STS-B and MRPC.

\subsection{Evaluation benchmarks}\label{sec:glue}

\subsubsection{GLUE}
The GLUE benchmark~\citep{wang2018glue} includes the following datasets:

\paragraph{MNLI} Multi-Genre Natural Language Inference is an entailment classification task~\citep{williams2018multi}.  The goal is to predict whether a given sentence {\it entails}, {\it contradicts}, or is {\it neutral} with respect to another.

\paragraph{QQP} Quora Question Pairs is a paraphrase detection task.  The goal is to classify whether two given questions have the same meaning.  The questions were sourced from the Quora question answering website~\citep{chen2018quora}.

\paragraph{QNLI} Question Natural Language Inference~\citep{wang2018glue} is a binary classification task which is derived from the Stanford Question Answering Dataset~\citep{rajpurkar2016squad}.  The task is to predict whether a sentence contains the answer to a given question.

\paragraph{SST-2} The Stanford Sentiment Treebank is a binary sentiment classification task, with content taken from movie reviews~\citep{socher2013recursive}.

\paragraph{CoLA} The Corpus of Linguistic Acceptability is a corpus of English sentences, each with a binary label denoting whether the sentence is linguistically acceptable~\citep{warstadt2019cola}.

\paragraph{STS-B} The Semantic Textual Similarity Benchmark is a sentence pair classification task.  The goal is to predict how similar the two sentences are in meaning, with scores ranging from 1 to 5~\citep{cer2017semeval}. 

\paragraph{MRPC} Microsoft Research Paraphrase Corpus is another sentence pair paraphrase detection task similar to QQP.  The sentence pairs are sourced from online news sources~\citep{dolan2005automatically}.

\paragraph{RTE} Recognizing Textual Entailment is a small natural language inference dataset similar to MNLI in content~\citep{bentivogli2009fifth}.

\subsubsection{SQuAD}
The SQuAD benchmark~\citep{rajpurkar2016squad}, \textit{i.e.}, Stanford Question Answering Dataset, is a reading comprehension dataset, consisting of questions on a set of Wikipedia articles, where the answer to each question is a segment of text from the corresponding passage, or the question might be unanswerable. 

\subsection{Technical details}\label{sec:technical}
% \input{tables/lr}
For each experiment, we sweep the learning rate in \{1e-4, 2e-4, 5e-4\} and the batch size in \{8, 16\} for QNLI, SST-2, CoLA, STS-B, MRPC, RTE, and \{16, 32\} for MNLI, QQP as well as SQuAD, and choose the settings with the highest accuracy on the validation set.
We use the same number of training epochs as BiBERT~\citep{qin2021bibert}, \textit{i.e.}, 50 for CoLA, 20 for MRPC, STS-B and RTE, 10 for SST-2 and QNLI, 5 for MNLI and QQP. 
We adopt the Adam optimizer with weight decay 0.01 and use 0.1 warmup ratio with linear learning rate decay. 

Our full precision checkpoints are taken from \url{https://textattack.readthedocs.io/en/latest/3recipes/models.html#bert-base-uncased}.

==> Binary Transformer (3)/figures/alpha.tex <==
\begin{wrapfigure}[9]{r}{0.58\textwidth}
    \centering
    \vspace{-1.2em}
    \includegraphics[width=1\linewidth]{figures/alpha_fig.pdf}
    \caption{The optimized scaling factor in \ours{}}
    \label{fig:alpha}
\end{wrapfigure}



==> Binary Transformer (3)/figures/paths.tex <==

\begin{wrapfigure}[16]{r}{0.5\textwidth}
    \vspace{-1em}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/paths_fig.pdf}
    \caption{MNLI-m accuracy on various distillation paths.  Each curve represents the sequence of models on a particular quantization schedule.}
    \label{fig:paths}
\end{wrapfigure}


==> Binary Transformer (3)/figures/whisky.tex <==
\begin{algorithm}[t]
\caption{\ours: Multi-distillation algorithm}
\label{alg:algorithm}
\small
\begin{algorithmic}[1]
\Require $\trainDataset, \devDataset$ \Comment{Training Data}
\Require $\model_0$ \Comment{Full-precision Model}
\Require $\mathbf{Q} = \{(b_w^1, b_a^1), \ldots, (b_w^k, b_a^k)\}$ \Comment{Quantization Schedule}
\State $\model_{\text{teacher}} \gets \ \model_0$
\For{$b_w^i, b_a^i$ in $\mathbf{Q}$}
\State $\model_{\text{student}} \gets \ \text{Quantize}(\model_{\text{teacher}}, b_w^i, b_a^i)$
\State $\text{KnowledgeDistill}(\model_{\text{student}}, \model_{\text{teacher}}, \trainDataset, \devDataset)$
\State $\model_{\text{teacher}} \gets \ \model_{\text{student}}$
\EndFor
\State \Return $\model_{\text{student}}$
\end{algorithmic}
\end{algorithm}


==> Binary Transformer (3)/tables/ablation.tex <==
\begin{table}[t]
\renewcommand\arraystretch{0.6}
\centering
\caption{Ablation study on the effects of each component on GLUE dataset without data augmentation.}
\label{tab:ablation_glue}
\setlength{\tabcolsep}{1.4mm}
{\fontsize{6.5pt}{\baselineskip}\selectfont
\begin{tabular}{llcccccccccccc}
\hline
\vspace{0.25pt}
& \textbf{Quant} & \begin{tabular}[c]{@{}c@{}}\textbf{MNLI}$_\text{-m/mm}$\end{tabular} & \textbf{QQP} & \textbf{QNLI} & \textbf{SST-2} & \textbf{CoLA} & \textbf{STS-B} & \textbf{MRPC} & \textbf{RTE} & \textbf{Avg.} \\ 
\hline
1 & BERT$_{\text{base}}$ & 84.9/85.5 & 91.4 & 92.1 & 93.2 & 59.7 & 90.1 & 86.3 & 72.2  & 83.9 \\ 
2 & BiBERT Baseline & 45.8/47.0 & 73.2 & 66.4 & 77.6 & 11.7 & 7.6 & 70.2 & 54.1 & 50.4 \\ 
3 & BiBERT & 66.1/67.5 & 84.8 & 72.6 & 88.7 & 25.4 & 33.6 & 72.5 & 57.4 & 63.2 \\ 
\hdashline[0.8pt/1pt]
4 & BinaryBERT (Our implementation) & 36.2/35.9 & 59.6 & 52.4 & 65.6 & 9.3 & 19.8 & 69.9 & 52.7 & 45.7 \\
5 & + Our simplied KD  & 37.7/37.3 & 59.5 & 56.8 & 73.4 & 4.1  & 24.8 & 70.8 & 57.0 & 48.0 \\
6 & + Our two-set binarization (Strong Baseline) & \textbf{57.4/59.1} & \textbf{68.3} & \textbf{64.7} & \textbf{81.0} & \textbf{18.2} & \textbf{24.7} & \textbf{71.8} & \textbf{56.7} & \textbf{55.3} \\ 
\hdashline[0.8pt/1pt] 
7 & + Elastic binarization (\ours{} $\ddag$) & 77.1/77.5 & 82.9 & 85.7 & 87.7 & 25.1 & 71.1 & 79.7 & 58.8 & 71.0 \\
8 & + Multi-Distillation (\ours{}) & \textbf{79.5/79.4} & \textbf{85.4} & \textbf{86.4} & \textbf{89.9} & \textbf{32.9} & \textbf{72.0} & \textbf{79.9} & \textbf{62.1} & \textbf{73.5}\\
\hline
\end{tabular}}
\end{table}



==> Binary Transformer (3)/tables/main_table.tex <==
\begin{table}[t]
\renewcommand\arraystretch{0.6}
\centering
\caption{Comparison of BERT quantization methods on the GLUE dev set. The E-W-A notation refers to the quantization level of embeddings, weights and activations. $\ddag$ denotes distilling binary models using full-precision teacher without using multi-distill technique in Section \ref{sec:whisky}. *Data augmentation is not needed for MNLI, QNLI, therefore results in the data augmentation section are identical to that without data augmentation for these datasets.}
\label{tab:glue}
\setlength{\tabcolsep}{1.4mm}
{\fontsize{6.5pt}{\baselineskip}\selectfont
\begin{tabular}{lcccccccccccc}
\hline
\vspace{0.25pt}
\textbf{Quant} & \begin{tabular}[c]{@{}c@{}}\textbf{\#Bits}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Size}$_\text{ (MB)}$\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{FLOPs}$_\text{ (G)}$\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{MNLI}$_\text{-m/mm}$\end{tabular} & \textbf{QQP} & \textbf{QNLI} & \textbf{SST-2} & \textbf{CoLA} & \textbf{STS-B} & \textbf{MRPC} & \textbf{RTE} & \textbf{Avg.} \\ 
\hline
BERT & 32-32-32 & 418 & 22.5 & 84.9/85.5 & 91.4 & 92.1 & 93.2 & 59.7 & 90.1 & 86.3 & 72.2  & 83.9 \\ 
\hdashline[0.8pt/1pt]
\multicolumn{3}{l}{\textit{Without data augmentation}} &&&&&&&&&& \\
Q-BERT & 2-8-8 & 43.0 & 6.5 & 76.6/77.0 & -- & -- & 84.6 & -- & -- & 68.3 & 52.7 & -- \\
Q2BERT & 2-8-8 & 43.0 & 6.5 & 47.2/47.3 & 67.0 & 61.3 & 80.6 & 0 & 4.4 & 68.4 & 52.7 &  47.7 \\
{TernaryBERT} & 2-2-8 & 28.0 & 6.4 & 83.3/83.3 & 90.1 & -- & -- & 50.7 & -- & 87.5 & 68.2 & -- \\
{BinaryBERT} & 1-1-8 & 16.5 & 3.1 & 84.2/84.7 & 91.2 & 91.5 & 92.6 & 53.4 & 88.6 & 85.5 & 72.2 & 82.7 \\
{BinaryBERT} & 1-1-4 & 16.5 & 1.5 & 83.9/84.2 & 91.2 & 90.9 & 92.3 & 44.4 & 87.2 & 83.3 & 65.3 & 79.9 \\
{BinaryBERT} & 1-1-2 & 16.5 & 0.8 & 62.7/63.9 & 79.9 & 52.6 & 82.5 & 14.6 & 6.5 & 68.3 & 52.7 &  53.7 \\
{BinaryBERT} & 1-1-1 & 16.5 & 0.4 & 35.6/35.3 & 66.2 & 51.5 & 53.2 & 0 & 6.1 & 68.3 & 52.7 & 41.0 \\
{BiBERT} & 1-1-1 & 13.4 & 0.4 & 66.1/67.5 & 84.8 & 72.6 & 88.7 & 25.4 & 33.6 & 72.5 & 57.4 & 63.2 \\
\hdashline[0.8pt/1pt]
\ours{} $\ddag$ & 1-1-4 & 13.4 & {1.5} & 83.6/84.4 & 87.8 & 91.3 & 91.5 & 42.0 & 86.3 & 86.8 & 66.4 & 79.5 \\
\ours{} $\ddag$ & 1-1-2 & 13.4 & {0.8} & 82.1/82.5 & 87.1 & 89.3 & 90.8 & 32.1 & 82.2 & 78.4 & 58.1 & 75.0\\
\ours{} $\ddag$ & 1-1-1 & 13.4 & {0.4} & 77.1/77.5 & 82.9 & 85.7 & 87.7 & 25.1 & 71.1 & 79.7 & 58.8 & 71.0\\ 
\ours{} & \textbf{1-1-1} & \textbf{13.4} & \textbf{0.4} & \textbf{79.5}/\textbf{79.4} & \textbf{85.4} & \textbf{86.4} & \textbf{89.9} & \textbf{32.9} & \textbf{72.0} & \textbf{79.9} & \textbf{62.1} & \textbf{73.5} \\
\hline
\multicolumn{3}{l}{\textit{With data augmentation}} &&&&&&&&&& \\
{TernaryBERT} & 2-2-8 &  28.0 & 6.4 & 83.3/83.3* & 90.1* & 90.0 & 92.9 & 47.8 & 84.3 & 82.6 & 68.4 & 80.3\\
{BinaryBERT} & 1-1-8 & 16.5 & 3.1 & 84.2/84.7* & 91.2* & 91.6 & 93.2 & 55.5 & 89.2 & 86.0 & 74.0 & 83.3 \\
{BinaryBERT} & 1-1-4 & 16.5 & 1.5 & 83.9/84.2* & 91.2* & 91.4 & 93.7 & 53.3 & 88.6 & 86.0 & 71.5 & 82.6 \\
{BinaryBERT} & 1-1-2 & 16.5 & {0.8}  & 62.7/63.9* & 79.9* & 51.0 & 89.6 & 33.0 & 11.4 & 71.0 & 55.9 & 57.6 \\
{BinaryBERT} & 1-1-1 & 16.5 & {0.4}  & 35.6/35.3* & 66.2* & 66.1 & 78.3 & 7.3 & 22.1 & 69.3 & 57.7 & 48.7 \\
{BiBERT} & 1-1-1 & 13.4 & 0.4 & 66.1/67.5* & 84.8* & 76.0 & 90.9 & 37.8 & 56.7 & 78.8 & 61.0 & 68.8 \\
\hdashline[0.8pt/1pt]
\ours{} $\ddag$ & 1-1-2 & 13.4 & {0.8}  & 82.1/82.5* & 87.1* &  88.8 & 92.5 & 43.2 & 86.3 & 90.4 & 72.9 & 80.4 \\
\ours{} $\ddag$ & 1-1-1 & 13.4 & {0.4}  & 77.1/77.5* & 82.9* &  85.0 & 91.5 & 32.0 & 84.1 & 88.0 & 67.5 & 76.0 \\
\ours{} & \textbf{1-1-1} & \textbf{13.4} & \textbf{0.4} & \textbf{79.5}/\textbf{79.4}* & \textbf{85.4}* & \textbf{86.5} & \textbf{92.3} & \textbf{38.2} & \textbf{84.2} & \textbf{88.0} & \textbf{69.7} & \textbf{78.0} \\
\hline
\end{tabular}}
\end{table}


==> Binary Transformer (3)/tables/progressive.tex <==
\begin{table}[h]
\centering
\caption{\ours{} vs. progressive distillation on selected GLUE tasks. Methods differ in the teacher model used and the model from which the student weights are initialized.}
\label{tab:progressive}
\setlength{\tabcolsep}{1.4mm}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\hline
\vspace{0.25pt}
\textbf{Method} & \textbf{Teacher} & \textbf{Initialization} & \textbf{MNLI}$_\text{-m/mm}$ & \textbf{QQP} & \textbf{QNLI} & \textbf{SST-2} & \textbf{CoLA} & \textbf{STS-B} & \textbf{MRPC} & \textbf{RTE} & \textbf{Avg.}\\ 
\hline
{BiBERT Distillation} & 32-32-32 & 32-32-32 & 77.0/77.2 & 83.1 & 84.1 & 89.7 & 31.3 & 60.1 & 75.5 & 56.7 & 69.7 \\ 
{Progressive} & 32-32-32 & 1-1-2 & 78.9/78.9 & 85.0 & 86.4 & 89.6 & 30.5 & \textbf{75.1} & \textbf{81.1} & 60.6 & 73.4 \\
\ours{} & \textbf{1-1-2} & \textbf{1-1-2} & \textbf{79.5/79.4} & \textbf{85.4} & \textbf{86.4} & \textbf{89.9} & \textbf{32.9} & 72.0 & 79.9 & \textbf{62.1} & \textbf{73.5} \\
\hline
\end{tabular}}
\end{table}





==> Binary Transformer (3)/tables/squad.tex <==
\begin{wraptable}[10]{r}{0.5\textwidth}
\vspace{-1.2em}
\centering
\caption{Comparison of BERT quantization methods on SQuADv1.1 dev set. Metrics are exact match and F1 score.}
\label{tab:squad}
\setlength{\tabcolsep}{2mm}
\resizebox{0.35\textwidth}{!}{
\begin{tabular}{lcc}
\hline
\vspace{0.25pt}
\textbf{Quant} & \begin{tabular}[c]{@{}c@{}}\textbf{\#Bits}\end{tabular} & \textbf{SQuADv1.1}$_\text{EM/F1}$ \\ 
\hline
BERT$_{\text{base}}$ & 32-32-32 & 82.6/89.7 \\ 
\hdashline[0.8pt/1pt]
{BinaryBERT} & 1-1-4 & 77.9/85.8 \\ 
{BinaryBERT} & 1-1-2 & 72.3/81.8 \\
{BinaryBERT} & 1-1-1 & 1.5/8.2 \\
{BiBERT} & 1-1-1 &  8.5/18.9 \\
\hdashline[0.8pt/1pt]
\ours{} & \textbf{1-1-1} & \textbf{63.1/74.9}\\
\hline
\end{tabular}}
\end{wraptable}

==> Binary Transformer (3)/tables/vs_biattention.tex <==
\begin{table}[h]
\centering
\caption{Two-set binarization scheme vs. Bi-Attention~\citep{qin2021bibert} on GLUE tasks. Methods differ in whether using $\rm{SoftMax}$ in attention and whether binarizing the $\rm{ReLU}$ output to \{0 ,1\}.}
\label{tab:vs_biattention}
\setlength{\tabcolsep}{1.4mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\hline
\vspace{0.25pt}
\textbf{Method} & \textbf{Attention} & \textbf{ReLU output} & \textbf{MNLI}$_\text{-m/mm}$ & \textbf{QQP} & \textbf{QNLI} & \textbf{SST-2} & \textbf{CoLA} & \textbf{STS-B} & \textbf{MRPC} & \textbf{RTE} & \textbf{Avg.}\\ 
\hline
Bi-Attention (w/o Softmax)& \{0, 1\} & \{-1, 1\}  & 48.1/50.0 & 60.1 & 60.6 & 78.8 & 14.0 & 22.3 & 68.4 & 58.1 & 51.3 \\
Binarize attention to \{0, 1\} (w/ Softmax) & \{0, 1\} & \{-1, 1\} & 51.9/52.6 & 76.2 & 60.5 & 79.6 & 11.6 & 18.1 & 70.6 & 55.6 & 53.0 \\
Two-set binarization scheme & \{0, 1\} & \{0, 1\}& 57.4/59.1 & 68.3 & 64.7 & 81.0 & 18.2 & 24.7 & 71.8 & 56.7 & 55.3 \\

\hline
\end{tabular}}
\end{table}

==> Binary Transformer (3)/tables/vs_reactnet.tex <==
\begin{table}[h]
\centering
\caption{Elastic binarization function vs. ReActNet~\citep{liu2020reactnet} learnable bias on GLUE tasks.}
\label{tab:vs_reactnet}
\setlength{\tabcolsep}{1.4mm}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\hline
\vspace{0.25pt}
\textbf{Method} & \textbf{MNLI}$_\text{-m/mm}$ & \textbf{QQP} & \textbf{QNLI} & \textbf{SST-2} & \textbf{CoLA} & \textbf{STS-B} & \textbf{MRPC} & \textbf{RTE} & \textbf{Avg.}\\ 
\hline
Our two-set binarization (Strong Baseline)& 57.4/59.1 & 68.3 & 64.7 & 81.0 & 18.2 & 24.7 & 71.8 & 56.7 & 55.3  \\ 
+ learnable scale & 76.5/76.8 & 82.7 & 85.1 & 88.1 & 26.6 & 62.3 & 74.3 & 58.1 & 69.2 \\
+ learnable scale and bias (BiT $\ddagger$)  & 77.1/77.5 & 82.9 & 85.7 & 87.7 & 25.1 & 71.1 & 79.7 & 58.8 & 71.0 \\
\hline
\end{tabular}}
\end{table}

==> backup/submission_supplementary_backup.tex <==
\section{Appendix}

\subsection{\ours{} vs. Progressive Distillation}\label{sec:progressive_ablation}
\input{tables/progressive}
Previous work has also recognized the importance of good initialization for binary model training, and proposed to perform distillation while progressively quantizing the student model \citep{zhuang2018towards, yang2019synetgy}.  Progressive distillation ensures a good initialization for the student model at each step.  However, in this approach the teacher model is fixed to the full precision model, which does not address the problem of teacher-student gap.  In Table \ref{tab:progressive} we compare \ours{} to a comparable implementation of progressive distillation, using the same quantization schedule, W32A32 $\rightarrow$ W1A2 $\rightarrow$ W1A1, as ours.  We keep the teacher model fixed, while re-initializing the student model from the latest quantized version at each step.  We see that using a quantized teacher model is helpful, especially in the high-data regime. However, our method can lag behind progressive distillation for small datasets such as STS-B and MRPC.

\subsection{Evaluation benchmarks}\label{sec:glue}

\subsubsection{GLUE}
The GLUE benchmark~\citep{wang2018glue} includes the following datasets:

\paragraph{MNLI} Multi-Genre Natural Language Inference is an entailment classification task~\citep{williams2018multi}.  The goal is to predict whether a given sentence {\it entails}, {\it contradicts}, or is {\it neutral} with respect to another.

\paragraph{QQP} Quora Question Pairs is a paraphrase detection task.  The goal is to classify whether two given questions have the same meaning.  The questions were sourced from the Quora question answering website~\citep{chen2018quora}.

\paragraph{QNLI} Question Natural Language Inference~\citep{wang2018glue} is a binary classification task which is derived from the Stanford Question Answering Dataset~\citep{rajpurkar2016squad}.  The task is to predict whether a sentence contains the answer to a given question.

\paragraph{SST-2} The Stanford Sentiment Treebank is a binary sentiment classification task, with content taken from movie reviews~\citep{socher2013recursive}.

\paragraph{CoLA} The Corpus of Linguistic Acceptability is a corpus of English sentences, each with a binary label denoting whether the sentence is linguistically acceptable~\citep{warstadt2019cola}.

\paragraph{STS-B} The Semantic Textual Similarity Benchmark is a sentence pair classification task.  The goal is to predict how similar the two sentences are in meaning, with scores ranging from 1 to 5~\citep{cer2017semeval}. 

\paragraph{MRPC} Microsoft Research Paraphrase Corpus is another sentence pair paraphrase detection task similar to QQP.  The sentence pairs are sourced from online news sources~\citep{dolan2005automatically}.

\paragraph{RTE} Recognizing Textual Entailment is a small natural language inference dataset similar to MNLI in content~\citep{bentivogli2009fifth}.

\subsubsection{SQuAD}
The SQuAD benchmark~\citep{rajpurkar2016squad}, \textit{i.e.}, Stanford Question Answering Dataset, is a reading comprehension dataset, consisting of questions on a set of Wikipedia articles, where the answer to each question is a segment of text from the corresponding passage, or the question might be unanswerable. 

\subsection{Technical details}\label{sec:technical}
% \input{tables/lr}
For each experiment, we sweep the learning rate in \{1e-4, 2e-4, 5e-4\} and the batch size in \{8, 16\} for QNLI, SST-2, CoLA, STS-B, MRPC, RTE, and \{16, 32\} for MNLI, QQP as well as SQuAD, and choose the settings with the highest accuracy on the validation set.
We use the same number of training epochs as BiBERT~\citep{qin2021bibert}, \textit{i.e.}, 50 for CoLA, 20 for MRPC, STS-B and RTE, 10 for SST-2 and QNLI, 5 for MNLI and QQP. 
We adopt the Adam optimizer with weight decay 0.01 and use 0.1 warmup ratio with linear learning rate decay. 

Our full precision checkpoints are taken from \url{https://textattack.readthedocs.io/en/latest/3recipes/models.html#bert-base-uncased}.
